Generate then Select: Open-ended Visual Question Answering Guided by World Knowledge

The open-ended Visual Question Answering (VQA) task requires AI models to jointly reason over visual and natural language inputs using world knowledge. Recently, pre-trained Language Models (PLM) such as GPT-3 have been applied to the task and shown to be powerful world knowledge sources. However, these methods suffer from low knowledge coverage caused by PLM bias -- the tendency to generate certain tokens over other tokens regardless of prompt changes, and high dependency on the PLM quality -- only models using GPT-3 can achieve the best result. To address the aforementioned challenges, we propose RASO: a new VQA pipeline that deploys a generate-then-select strategy guided by world knowledge for the first time. Rather than following the de facto standard to train a multi-modal model that directly generates the VQA answer, RASO first adopts PLM to generate all the possible answers, and then trains a lightweight answer selection model for the correct answer. As proved in our analysis, RASO expands the knowledge coverage from in-domain training data by a large margin. We provide extensive experimentation and show the effectiveness of our pipeline by advancing the state-of-the-art by 4.1% on OK-VQA, without additional computation cost. Code and models are released at http://cogcomp.org/page/publication_view/1010

==> tables/implementation_detail.tex <==

\begin{table*}[]
\begin{tabular}{llllllllll}
Model      & Size  & no. para & machine & no. GPU & Time     & GPU hours & lr       & total step & optim \\
KAT        & large & 770M   & v100    & 8     & 3.75 hrs & 30        & 3.00E-05 & 8000       & adamw \\
Unified-QA & large & 770M   & v100    & 8     & 1.75 hrs & 14        & 5.00E-05 & 8000       & adamw \\
ClipCap    &       &        & v100    & 1     & 6 hrs    & 6         &          &            &      
\end{tabular}
\caption{Implementation details}
\end{table*}
